A Finite Element Configuration Interaction Method for Wigner Localization

The Wigner localization is an electron phase at low densities when the electrons are sharply localized around equilibrium positions. The simulation of the Wigner localization phenomenon requires careful treatment of the many-body correlations, as the electron-electron interaction dominates the system. This work proposes a numerical algorithm to study the electron ground states of the Wigner molecules. The main features of our algorithm are three-fold: (i) a finite element discretization of the one-body space such that the sharp localization can be captured; (ii) a good initial state obtained by exploiting the strongly correlated limit; and (iii) a selected configuration interaction method by choosing the Slater determinants from (stochastic) gradients. Numerical experiments for some typical one-dimensional quantum wires and two-dimensional circular quantum dots are provided to show the efficiency of our algorithm.

==> bak/bak-main.tex <==
% BAK

Therefore, the FCI variational space $\mathcal{V}$ spanned by these basis functions is 
\begin{eqnarray*}
 \label{Nbody_span}
 \mathcal{V}:=\mathrm{span}\big\{|\phi_{i_1}\chi_{s_1}\phi_{i_2}\chi_{s_2}\cdots\phi_{i_N}\chi_{s_N}\rangle\big\}_{\substack{i_1,\cdots,i_N\in\{1,\cdots,n_{orb}\},\,s_1,\cdots,s_N\in\{0,1\}}}
\end{eqnarray*}
with $\mathrm{dim}(\mathcal{V})=\binom{2n_{orb}}{N}=:N_\mathrm{FCI}$. It is important to remember that the indices $i_a,s_a$ $(a = 1,\cdots,N)$ can not be chosen arbitrarily, due to the permutation symmetry. A simple way of indexing is to restrict 
\begin{eqnarray*}
 i_a+Ns_a<i_b+Ns_b\quad if \, 1\leq a<b\leq N,
\end{eqnarray*}
 which will be used in our practical implementations.
 We denote the index set as $\mathcal{I}$,
 \begin{eqnarray}
 \label{index}
	\begin{array}{ll}
	 \mathcal{I}=\big\{(i_1,s_1,\cdots,i_N ,s_N)|i_a\in\{1,\cdots,n_{orb}\},\,s_a\in\{0,1\},\,a=1,\cdots,N,\\
	\hspace{30pt}i_a+Ns_a<i_b+Ns_b,\, if \, 1\leq a<b\leq N\big\},
	\end{array}
 \end{eqnarray}
with $|\mathcal{I}|=N_\mathrm{FCI}$.

Then, the ground state wave function could be discretized in $\mathcal{V}$, and could be written as
 \begin{eqnarray}
 \label{linspan}
	\Psi=\sum_{\pmb{i}\in\mathcal{I}}c_{\pmb{i}} \Phi_{\pmb{i}} .
 \end{eqnarray}
Substituting (\ref{linspan}) into (\ref{WigCSchrodinger}), one obtains the matrix representation \cite{Sherrill1999}
\begin{eqnarray}
 \label{matrixform}
	H^{(\alpha)} \pmb{c}=E_\alpha{S}\pmb{c},
\end{eqnarray}
where the Hamiltonian operator $\hat{H}_\alpha$ is replaced by a many-body Hamiltonian matrix $H^{(\alpha)}$ and $\Psi$ is replaced by a column vector of coefficients $\pmb{c}$. 
The matrix elements of the Hamiltonian are given by $H^{(\alpha)}_{{\pmb{i}}{\pmb{j}}}= \langle\Phi_{\pmb{i}}|\hat{H}_\alpha|\Phi_{\pmb{j}}\rangle$, and ${S}$ is the overlap matrix with elements ${S}_{{\pmb{i}}{\pmb{j}}}=\langle\Phi_{\pmb{i}}|\Phi_{\pmb{j}}\rangle$. 
Eqn (\ref{matrixform}) is known as the FCI generalized eigenvalue problem, the smallest eigenvalue is the ground state energy and the corresponding eigenvector is the ground state wave function. 


\begin{algorithm}[H]
	\caption{Initial state for Wigner crystals} %算法的名字
	\hspace*{0.02in} {\bf Input:} %算法的输入， \hspace*{0.02in}用来控制位置，同时利用 \\ 进行换行
	Positive integer $M_1, M_2<n_{orb}$.\\
	\hspace*{0.02in} {\bf Output:} %算法的结果输出
	Initial vector $\pmb{c}_\mathrm{wig}$ for Wigner crystals.

	\begin{algorithmic}[1]
	    \State Solve (\ref{nonlineq}) to obtain $\{\rr_i\}:=\{\rr_{i_1},\dots, \rr_{i_{M_1}}\}\subset[-L,L]^d$ which belong to $U$;
		\For{$k=1,\cdots,N$} % For 语句，需要和EndFor对应
		\For{$l=1,\cdots,M_1$}
		\State $j_{k_l}=\argmin\limits_{j}dist(\rr_{i_l},X_j)$, where $dist(\rr_{i_l},X_j) = inf\{|\rr_{i_l}-\mathbf{x}_j|:\mathbf{x}_j\in X_j\}$. %where $X_j$ is the domain of $\phi_j$ ;
		\State $i_{k _l}^1,\cdots,i_{k _l}^{M2}=\argmin\limits_{j_1,\dots,j_{M_2}}\sum_{\ell=1}^{M_2}dist(X_{j_{k_l}},X_{j_\ell})$ and $i_{k _l}^1<\cdots<i_{k _l}^{M2}$, where
		\Statex \hspace{37pt}$dist(X_{j_{k_l}},X_{j_\ell}) = inf\{dist(\mathbf{x}_{j_{k_l}},X_{j_\ell}):\mathbf{x}_{j_{k_l}}\in X_{j_{k_l}}\}$.
		\State $R_{k_l}=\{(i_{k _l}^1,0),\cdots,(i_{k _l}^{M2},0),(i_{k _l}^1,1),\cdots,(i_{k _l}^{M2},1)\}$.
        \EndFor
        \State{\bf end for}
        \EndFor
        \State{\bf end for}
        \For {$l=1,\cdots,M_1$}
        \State For each $(i_{k_l},s_{k_l})\in R_{k_l}$, $k=1,\cdots,N$: Sort $(i_{1_l},s_{1_l},\cdots,i_{N_l},s_{N_l})$ in ascending order 
        \Statex \hspace{18.5pt}based on $i_{k_l}+N s_{k_l}$, denoted as $\pmb{i}_{R_l}$.
        \State Check whether $\pmb{i}_{R_l}\in\mathcal{I}$. If yes, $\pmb{i}_{R_l}\in\mathcal{I}_\mathrm{wig}$,
        \EndFor
        \State{\bf end for}
        \State Generate $H^{(\alpha)}_\mathrm{wig}\in\mathbb{R}^{N_\mathrm{wig}\times N_\mathrm{wig}}$ and $S_\mathrm{wig}\in\mathbb{R}^{N_\mathrm{wig}\times N_\mathrm{wig}}$ from $\mathcal{I}_\mathrm{wig}$.
        \State Solve $H^{(\alpha)}_\mathrm{wig} \pmb{c}_\mathrm{wig}=E_\mathrm{wig}{S_\mathrm{wig}}\pmb{c}_\mathrm{wig}$.
	\end{algorithmic}
\end{algorithm}


Firstly, we need to predict the positions of peaks of the Dirac distribution in the SCE system, the corresponding ground state energy is
\begin{eqnarray*}
	\begin{aligned}
		E_0 := &\lim_{\alpha\to0}E_\alpha= \min\limits_{\Psi\in \A}\langle\Psi|\hat{V}_\mathrm{ee}+\hat{V}_\mathrm{ext}|\Psi\rangle
	 \notag \\
	 =: &\min\limits_{\Psi\in \A} E_0[\Psi]=E_0[\Psi^{\mathrm{SCE}}].
	\end{aligned}
\end{eqnarray*}
Since $|\Psi^{\mathrm{SCE}}|^2$ is only determined by spatial variables, write
\begin{eqnarray*}
|\Psi^{\mathrm{SCE}}|^2=|\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2,
\end{eqnarray*}
and obtain
\begin{eqnarray*}
E_0 =\int|\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2\Bigg\{\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\rr_i-\rr_j|}+\sum_{i=1}^{N} v(\rr_i)\Bigg\}\rm d\rr_1\dots \rm d\rr_N.
\end{eqnarray*}
Let $\Omega\subset\mathbb{R}^d$ be the spatial domain for one electron. We consider $\Omega$ is compact and $v(\rr)\in C^\infty(\Omega)$ here. $F$ is defined as
\begin{eqnarray}
\label{F}
F(\rr_1,\dots,\rr_N) := \sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\rr_i-\rr_j|}+\sum_{i=1}^{N} v(\rr_i),\,\{\rr_i\} \subset\Omega,
\end{eqnarray}
and
\begin{eqnarray}
\label{W}
W := \min_{\substack{{\{\rr_i\}}\subset\Omega}}
F(\rr_1,\dots,\rr_N),
\end{eqnarray}
then
\begin{eqnarray*}
E_0\geq  \int |\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2W \rm d\rr_1\dots \rm d\rr_N =W.
\end{eqnarray*}
If we assume ${\{\tilde{\rr}_i\}}_{i=1}^N\in U$, where
\begin{eqnarray}
\label{U}
U := \{\{\rr_i\}_{i=1}^N\subset\Omega^N|\{\rr_i\}_{i=1}^N \,\, \mathrm{are \,\, minimizers \,\, of} \,\, F\},
\end{eqnarray}
and there is a $\tilde{\Psi}$ that satisfies 
\begin{eqnarray*}
|\tilde{\Psi}(\rr_1,\dots,\rr_N)|^2=\dfrac{1}{N!}\sum_{\Pa}\delta(\rr_1-\tilde{\rr}_{\Pa(1)})\times\dots\times\delta(\rr_N-\tilde{\rr}_{\Pa(N)}).
\end{eqnarray*}
It follows that

\begin{eqnarray*}
	\begin{aligned}
		E_0\leq E_0[\tilde{\Psi}]=&\int|\tilde{\Psi}(\rr_1,\dots,\rr_N)|^2\Bigg\{\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\rr_i-\rr_j|}+\sum_{i=1}^{N} v(\rr_i)\Bigg\}\rm d\rr_1\dots \rm d\rr_N\notag\\
		=&\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\tilde{\rr}_i-\tilde{\rr}_j|}+\sum_{i=1}^{N} v(\tilde{\rr}_i)\\
		=&W,
	\end{aligned}
\end{eqnarray*}
then
\begin{eqnarray*}
E_0=E_0[\tilde{\Psi}]=W.
\end{eqnarray*}
The conclusion is that the minimizers ${\{\tilde{\rr}_i\}}_{i=1}^N$ are the positions of distribution peaks in the SCE system.

The crucial problem is how to solve (\ref{W}). Here we consider $\Omega=[-L,L]^d$, $d\in\{1,2\}$, denote $\rr_i = (r_i^1,\dots,r_i^d)$, 
calculate the partial derivatives of $F$ in (\ref{F}),
\begin{eqnarray*}
\label{deriv}
\frac{\partial F}{\partial r_i^l} = -\sum_{j\neq i}^{N}\frac{r_i^\ell-r_j^\ell}{|\rr_i-\rr_j|^3}+\frac{\partial v_\mathrm{ext}(\rr_i)}{\partial r_i^l}\,\,(\ell = 1,\dots d,\,i=1,\dots,N).
\end{eqnarray*}
Let $ F_{r_i^\ell}=0$ $(\ell = 1,\dots d,\,i=1,\dots,N)$, get the nonlinear equations
\begin{eqnarray}
\label{nonlineq}
-\sum_{j\neq i}^{N}\frac{r_i^\ell-r_j^\ell}{|\rr_i-\rr_j|^3}+\frac{\partial v_\mathrm{ext}(\rr_i)}{\partial r_i^l}=0\,\,(\ell = 1,\dots d,\,i=1,\dots,N).
\end{eqnarray}
(\ref{nonlineq}) could be approximately solved by numerical methods, such as Newton method. We only choose the ones for which have the minimum value of $F$ in (\ref{F}). 



The crucial problem is how to solve (\ref{W}). Here we consider $\Omega=[-L,L]^d$, $d\in\{1,2\}$, denote $\rr_i = (r_i^1,\dots,r_i^d)$, 
calculate the partial derivatives of $F$ in (\ref{F}),
\begin{eqnarray*}
\label{deriv}
\frac{\partial F}{\partial r_i^l} = -\sum_{j\neq i}^{N}\frac{r_i^\ell-r_j^\ell}{|\rr_i-\rr_j|^3}+\frac{\partial v_\mathrm{ext}(\rr_i)}{\partial r_i^l}\,\,(\ell = 1,\dots d,\,i=1,\dots,N).
\end{eqnarray*}
Let $ F_{r_i^\ell}=0$ $(\ell = 1,\dots d,\,i=1,\dots,N)$, get the nonlinear equations
\begin{eqnarray}
\label{nonlineq}
-\sum_{j\neq i}^{N}\frac{r_i^\ell-r_j^\ell}{|\rr_i-\rr_j|^3}+\frac{\partial v_\mathrm{ext}(\rr_i)}{\partial r_i^l}=0\,\,(\ell = 1,\dots d,\,i=1,\dots,N).
\end{eqnarray}


Firstly, we need to predict the positions of peaks of the Dirac distribution in the SCE system, the corresponding ground state energy is
\begin{eqnarray*}
	\begin{aligned}
		E_0 := &\lim_{\alpha\to0}E_\alpha= \min\limits_{\Psi\in \A}\langle\Psi|\hat{V}_\mathrm{ee}+\hat{V}_\mathrm{ext}|\Psi\rangle
	 \notag \\
	 =: &\min\limits_{\Psi\in \A} E_0[\Psi]=E_0[\Psi^{\mathrm{SCE}}].
	\end{aligned}
\end{eqnarray*}
Since $|\Psi^{\mathrm{SCE}}|^2$ is only determined by spatial variables, write
\begin{eqnarray*}
|\Psi^{\mathrm{SCE}}|^2=|\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2,
\end{eqnarray*}
and obtain
\begin{eqnarray*}
E_0 =\int|\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2\Bigg\{\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\rr_i-\rr_j|}+\sum_{i=1}^{N} v(\rr_i)\Bigg\}\rm d\rr_1\dots \rm d\rr_N.
\end{eqnarray*}


then
\begin{eqnarray*}
E_0\geq  \int |\Psi^{\mathrm{SCE}}(\rr_1,\dots,\rr_N)|^2W \rm d\rr_1\dots \rm d\rr_N =W.
\end{eqnarray*}

It follows that

\begin{eqnarray*}
	\begin{aligned}
		E_0\leq E_0[\tilde{\Psi}]=&\int|\tilde{\Psi}(\rr_1,\dots,\rr_N)|^2\Bigg\{\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\rr_i-\rr_j|}+\sum_{i=1}^{N} v(\rr_i)\Bigg\}\rm d\rr_1\dots \rm d\rr_N\notag\\
		=&\sum_{i=1}^{N-1}\sum_{j=i+1}^N \frac{1}{|\tilde{\rr}_i-\tilde{\rr}_j|}+\sum_{i=1}^{N} v(\tilde{\rr}_i)\\
		=&W,
	\end{aligned}
\end{eqnarray*}


Consider the limit $\alpha\to 0$ of infinitely strong repulsion, which be called the ‘‘strictly correlated electrons" (SCE) limit,
\begin{eqnarray}
\label{SCE}
\lim_{\alpha\to0}E_\alpha=\lim_{\alpha\to0}\min\limits_{\Psi\in \A}\langle\Psi|\ham_\alpha|\Psi\rangle=\min\limits_{\Psi\in \A}\langle\Psi|V_\mathrm{ee}+V_\mathrm{ext}|\Psi\rangle.
\end{eqnarray}
In this system, the electrons are strictly correlated, in the sense that the position of one of them determines the positions of the others\cite{Christian14}.
And the limiting minimizing
wave function $\Psi^{\mathrm{SCE}}$ dosen't depend on the spin variables $\st_1,\dots,\st_N$, and, since the limit is classical, we can only determine $|\Psi^{\mathrm{SCE}}|^2$, which, in terms of the spatial variables $\rr_1,\dots,\rr_N$, is a Dirac-type distribution,
describing electrons with strictly correlated positions \cite{Paola10}. And the
Dirac-type distribution could be described by the finite elements well.



We observe by a direct calculation that
\begin{eqnarray*}
\label{energyscaling}
\big\langle\Psi_\alpha \big| \ham \big| \Psi_\alpha \big\rangle = \alpha \big\langle \Psi \big| \hama \big| \Psi\big\rangle .
\end{eqnarray*}
%
Consequently, $\Psi_\alpha$ is the ground state of $\ham$ if and only if $\Psi$ is the ground state of $\hama$.


Let $\alpha>0$ be a scaling parameter.
For a given wavefunction $\Psi \in\A$, we consider the scaled wavefunction
\begin{eqnarray}
\label{scaling}
\Psi_\alpha(\rr_1,\st_1, \dots,\rr_N,\st_N):=\alpha^{\frac{Nd}{2}}\Psi(\alpha\rr_1,\st_1, \dots,\alpha\rr_N,\st_N) 
\qquad \rr_i\in ,
% \qquad (\alpha>0)
\end{eqnarray}
where $\Omega_{\alpha} = \{\rr\in\R^d~:~\alpha\rr\in\Omega\}$ and the prefactor $\alpha^{\frac{Nd}{2}}$ guarantees that $\Psi_\alpha$ still satisfies the normalization constraint in ${\A}$.
%
For $\Psi\in\A$, the corresponding one-electron density is given by
\begin{eqnarray}
\label{density}
\rho_{\Psi}(\rr)= N\sum_{\st_1,\cdots,\st_N\in\Z_2}\int \big| \Psi(\rr,\st_1, \dots,\rr_N,\st_N) \big|^2 \rm d\rr_2\dots ~{\rm d}\rr_N .
\end{eqnarray}
For simplicity of presentations, we will drop the subscript and denote the density by $\rho$ whenever it is clear from the context.
%
The corresponding one-electron density becomes 
\begin{eqnarray*}
\rho_{\Psi_\alpha}(\rr) = \alpha^d \rho_{\Psi}(\alpha \rr).
\end{eqnarray*}
% Notice that $\Psi_\alpha \in L^2\big( (\frac{\Omega}{\alpha} \times\mathbb{Z}_2)^N;\mathbb{C}\big)$, it has the average electron density 
We immediately see that $\Bar{\rho}_{{\Psi_\alpha}} = \alpha^d\Bar{\rho}_{\Psi}$, which together with \eqref{rs} gives the Wigner-Seitz radius $\rsa$ of the scaled system
\begin{eqnarray*}
\label{rsa}
\rsa = \frac{1}{\alpha} \rs .
\end{eqnarray*}
%
That is, large values of scaling parameters $\alpha$ correspond to concentrated systems with high density and small values of $\alpha$ correspond to diluted systems low density. 

We will then perform a scaling argument by following \cite{Chen2015,Levy1985} to access different regimes by simply changing one scaling parameter $\alpha$, which we will show is essentially determined by the Wigner-Seitz radius $\rs$. 

Then to study the transition/crossover of the Wigner crystallization, we can govern the system by tuning the parameter $\alpha$.
%
More precisely, when $\alpha$ is small, the system lies in the low-density regimes, for which the Coulomb energy dominates over the kinetic energy. 
In this case, the electrons localize around particular positions on the domain that minimize their energy.
In contrast, when $\alpha$ is large, the system has high-density and the kinetic energy become dominant. 
In this case, the electrons are weakly correlated and the mean-field based methods can get good approximations.



The selected CI methods rely on the same principle as the usual CI approaches, except that determinants aren’t chosen a priori based on an occupation or excitation criterion, but selected on the fly among the entire set of determinants based on their estimated contribution to the FCI wave function. 
It has been noticed long ago that, even inside a predefined subspace of determinants, only a small number significantly contributes to the wave function \cite{Anderson18,Bytautas09}. 
Therefore, an on the fly selection of determinants is a rather natural idea that has been proposed \cite{Lu2019}.




\begin{itemize}
  \item [1.] 
  Find the iteration set $\K^{\lo}$ according to the magnitude of $\pmb{g}^{\la}$ which is the approximation of $\nabla f(\pmb{c}^{\la})$, and add $\K^{\lo}$ to $\J^{\la}$ to obtain $\J^{\lo}$.
  \item [2.]
  Determine the stepsize $\beta$ by the line search, and update $\pmb{c}^{\lo} = \pmb{c}^{\la} + \beta \pmb{g}_{\K^{\lo}}^{\la}$, where $\pmb{g}^{\la}_{\K^{\lo}}:=\sum_{\is\in\K^{\lo}}\pmb{g}^{\la}_{\is}\pmb{e}_{\is}$ with $\pmb{e}_{\is}$ denotes the indicator vector of $\is$.
  \item [3.]
  For next iteration, update $\pmb{g}^{\lo}$ with a compression strategy which saves memory resource.
  \item [4.] 
  Calculate $f(\pmb{c}^{\lo})$ as the ground state energy estimator.
\end{itemize}
We stop the iteration when some stopping criteria are reached. 

More general methods include monitoring the decay of the Rayleigh quotient and the cumulated updated values across a few iterations \cite{Lu2019}.


\begin{eqnarray*}
\K^{\lo} := \Big\{\is_1,\dots,\is_\kk :~ |\pmb{g}^{\la}_{\is_1}|\geq\cdots\geq|\pmb{g}^{\la}_{\is_\kk}|\geq|\pmb{g}^{\la}_{\jt}|,
~ \forall~\jt \in\I\setminus\{\is_1,\dots,\is_\kk\}\Big\}.
\end{eqnarray*}


\begin{multline}
\label{select}
\qquad\qquad\K^{\lo} := \Big\{\is_1,\dots,\is_\kk\in\I_H(\La^{\la}) :~ |\pmb{g}^{\la}_{\is_1}|\geq\cdots\geq|\pmb{g}^{\la}_{\is_\kk}|\geq|\pmb{g}^{\la}_{\jt}|,
\\
\forall~\jt \in\I_H(\La^{\la})\setminus\{\is_1,\dots,\is_\kk\}\Big\}.\qquad
\end{multline}
Since the number of the $H$-connected determinants of $\La^{\la}$ grows exponentially with $N$, when treat more than five electrons, we randomly check part of $\I_H(\La^{\la})$ to save computational cost.


The gradient of $f$ is given by
\begin{eqnarray*}
\label{gradient}
\nabla f(\pmb{c})=\dfrac{2\Ha\pmb{c}}{\pmb{c}^\top S\pmb{c}}-\dfrac{2S\pmb{c}(\pmb{c}^\top  \Ha\pmb{c})}{(\pmb{c}^\top S\pmb{c})^2}.
\end{eqnarray*}

We begin by setting $\I_\delta$ as the initial selected space $\J^{(0)}$, $\pmb{c}_{\I_\delta}$ as the initial state $\pmb{c}^{(0)}$.

After adding $\K^{\lo}$ to $\J^{\la}$, i.e., 
\begin{eqnarray}
\label{setupdate}
\J^{\lo}=\J^{\la}\cup\K^{\lo}, 
\end{eqnarray}
we need to find the stepsize of the determinants in $\K^{\lo}$ to update $\pmb{c}^{\la}$. Step 2 determines the stepsize by the exact line search along that direction so to decrease the objective function value by the largest amount.


Denoting the update as $\beta $,
\begin{eqnarray}
\label{update}
\beta =  \argmin\limits_{\tilde{\beta }\in\mathbb{R}}f(\pmb{c}^{\la}+\tilde{\beta }\pmb{g}^{\la}_{\K^{\lo}}).
\end{eqnarray}
Solving the minimization problem \eqref{update} is equivalent to finding roots of $h'(\tilde{\beta })=0$ with $h(\tilde{\beta })=f(\pmb{c}^{\la}+\tilde{\beta }\pmb{g}^{\la}_{\K^{\lo}})$, which is a quadratic equation in $\tilde{\beta }$. Given the update $\beta $, we can update $\pmb{c}^{\lo}$ as

\begin{eqnarray}
\label{wfupdate}
\pmb{c}^{\lo}_{\is} =
\left\{ \begin{array}{ll}
	\pmb{c}^{\la}_{\is}, &{\is}\notin {\K}^{\lo},\\
	\pmb{c}^{\la}_{\is} +\beta\pmb{g}^{\la}_{\is} ,\quad &{\is}\in {\K}^{\lo},\\
\end{array} \right.
\end{eqnarray}
where $\pmb{c}|_{\J^{\lo}} \neq 0$.      



future iterations, we also need to update
\begin{eqnarray}
\label{gradientaprx}
\pmb{g}^{\lo}:= \dfrac{2\pmb{b}^{\lo}}{(\pmb{c}^{\lo})^\top S \pmb{c}^{\lo}}-\dfrac{2\pmb{d}^{\lo}(({\pmb{c}^{\lo}})^\top \Ha \pmb{c}^{\lo})}{(({\pmb{c}^{\lo}})^\top S \pmb{c}^{\lo})^2},
\end{eqnarray}
where 
\begin{eqnarray*}
\pmb{b}^{\lo}:= \Ha\pmb{c}^{\lo}= \pmb{b}^{\la}+\beta  \Ha\pmb{g}^{\la}_{\K^{\lo}}\quad \mathrm{and}\quad \pmb{d}^{\lo}:= S\pmb{c}^{\lo}= \pmb{d}^{\la}+\beta  S\pmb{g}^{\la}_{\K^{\lo}}.
\end{eqnarray*}
We first compute $\pmb{b}^{\lo}$ and $\pmb{d}^{\lo}$,
since the exact update for them will waste computational and memory cost on unimportant determinants, the compression strategy has been proposed, i.e.,
\begin{eqnarray}
\label{compress}
\pmb{b}_{\is}^{\lo} =
		\left\{ \begin{array}{ll}
			\pmb{b}_{\is}^{\la}+\beta (\Ha\pmb{g}^{\la}_{\K^{\lo}})_{\is},\quad &\pmb{b}_{\is}^{\la}\ne0\quad \rm{or} \quad|\beta (\Ha\pmb{g}^{\la}_{\K^{\lo}})_{\is}|>\varepsilon,\\
			0,&\mathrm{else},
\end{array} \right.
\end{eqnarray}
where $\varepsilon > 0$ is a predefined tolerance, and treat $\pmb{d}^{\lo}$ as the same way. To guarantee the correctness and increase the numerical stability of the algorithm, we recalculate the $\K^{\lo}$-th entries in $\pmb{b}^{\lo}$ and $\pmb{d}^{\lo}$ \cite{Lu2019},
\begin{eqnarray}
\label{recal}
\pmb{b}_{\is}^{\lo}=(\Ha\pmb{c}^{\lo})_{\is}\quad\mathrm{and}\quad\pmb{d}_{\is}^{\lo}=(S\pmb{c}^{\lo})_{\is},\qquad \is\in\K^{\lo}.
\end{eqnarray}
The recalculation could improve the accuracy of the determinant-select (\ref{select}) and line search (\ref{update}) in the following iterations, and also provide accurate calculations of ${\pmb{c}^{\lo}})^\top \Ha \pmb{c}^{\lo}$ and ${\pmb{c}^{\lo}})^\top S \pmb{c}^{\lo}$,
\begin{eqnarray}
\label{energyH}
({\pmb{c}^{\lo}})^\top \Ha \pmb{c}^{\lo}=({\pmb{c}^{\la}})^\top \Ha \pmb{c}^{\la}+2\beta(\pmb{g}^{\la}_{\K^{\lo}})^\top\pmb{b}^{\lo}-\beta^2(\pmb{g}^{\la}_{\K^{\lo}})^\top\Ha\pmb{g}^{\la}_{\K^{\lo}},
\end{eqnarray}
\begin{eqnarray}
\label{energyS}
({\pmb{c}^{\lo}})^\top S \pmb{c}^{\lo}=({\pmb{c}^{\la}})^\top S \pmb{c}^{\la}+2\beta(\pmb{g}^{\la}_{\K^{\lo}})^\top\pmb{d}^{\lo}-\beta^2(\pmb{g}^{\la}_{\K^{\lo}})^\top S\pmb{g}^{\la}_{\K^{\lo}}.
\end{eqnarray}
And the Rayleigh quotient $f(\pmb{c})$ can be maintained accurately for $\pmb{c}^{\lo}$, which is used as the estimator of the ground state energy.

By varying $\varepsilon$, we can obtain accurate results without wasting memory cost on the small terms. We choose $\varepsilon$ by following CD-FCI \cite{Lu2019}.

In 1D systems, we first compare the performance of HF as initial state with semi-classical limit on a four particles system to illustrate the high efficiency of our algorithm in dealing with the strongly correlated systems. Then, we present the evolution of one-electron density from weak to strong correlation.


Firstly, two initial states are tested for four electrons on a sequence of $\alpha$. Figure \ref{fig:example1d:err} shows the energy error against the iteration number. Here the energy error is defined as the difference between the ground state energy calculated by algorithms at current iteration and the exact ground state energy calculated by FCI. We notice that, when $\alpha=10$ and $\alpha = 1$, semi-classical limit converges faster at the beginning, with iteration, the convergence rate decreases, and the error is larger than HF. When $\alpha = 0.1$, the error of semi-classical limit is smaller all the time. 
So when simulating WCs, semi-classical limit is much better. It has lower initial energy and faster convergence to the exact ground state. In addition, comparing the three pictures, one can find that 
the smaller $\alpha$ has lower initial energy and smaller error after same iterations. So the stronger the correlation, the fewer iterations needed to reach convergence.


After demonstrating the high efficiency of our method for simulating WCs, we compute the densities for $N = 4, 6$. The results for different values of $\alpha$ are presented in Figure \ref{fig:example1d:density}, where $\alpha = 10,1$ calculated by HF, $\alpha = 0.1$ by Algorithm 3.2. It can be seen that for weak correlation $\alpha = 10$, the number of peaks is half of the number of electrons. As interaction increases, for $\alpha = 1$, $N$ peaks appear, but with a small peak-valley ratio. As $\alpha$ further decreases, the peak-valley ratio increases as the minima of density is tend to zero and the peaks gradually approaches the solid symbols, which means the Wigner crystallization gradually appears. 


In 2D numerical experiments, we show the evolution of density, and use semi-classical limit to simulate some typical systems with Wigner localization. We consider quantum dots laterally confined by different parabolic potential, that is, $\Omega = [-5,5] ^ 2$, $v_{\rm{ext}}(x,y) = \omega (x^2 + y^2)$ with $\omega > 0$. Actually, the parabolic potential makes electrons confined on circular-symmetric quantum dots, and the size of circle is decided by the value of $\omega$. For Algorithm 3.2, the compression threshold $\varepsilon = 5\times10^{-7}$ and the mesh size $M_h = 30\times 30$. In our calculation, we take $N = 3,4,5,6$ and $\alpha = 0.1, 0.4, 1.6$, corresponding to values $\rs$ between $\sim$ ? and ?.

We simulate the weak-to-strong correlation transition of 3 electrons with $\omega = 0.2$ by controlling the value of $\alpha$. The evolution of density is presented in Figure \ref{fig:example2d:cross-over}, where $\alpha = 1.6$ calculated by HF, $\alpha = 0.4, 0.1$ by semi-classical limit. We see that when $\alpha = 1.6$, the density is dumbbell shaped and concentrated on the middle area. As interaction increases, for $\alpha = 0.4$, a thick ring occurs with smooth density. For stronger correlation $\alpha = 0.1$, the density becomes much sharper, forming a very thin ring centered at the origin. 


To observe the Wigner localization of different particles, the densities of $N$ = 4, 5, 6 for $\alpha$ = 0.1 are depicted in Figure \ref{fig:example2d:density}. And we save computational and memory cost by controlling the value of $\omega$, set $\omega = 0.8$ for $N = 4$, $\omega = 1$ for $N = 5$, $\omega = 2$ for $N = 6$. Since the densities concentrate on the middle area, we only draw the densities in $\Omega=[-3,3]^2$. For $N$ = 4, 5, there is a sharp ring like $N = 3$. For $N$ = 6, the density consists of a peak in the origin (integrating to one particle) and a sharp ring surrounding it (which integrates to five particles).


